Finding Short Signals in Long Irregular Time Series with Continuous-Time Attention Policy Networks

Irregularly-sampled time series (ITS) are native to high-impact domains like healthcare, where measurements are collected over time at uneven intervals. However, for many classification problems, only small portions of long time series are often relevant to the class label. In this case, existing ITS models often fail to classify long series since they rely on careful imputation, which easily over- or under-samples the relevant regions. Using this insight, we then propose CAT, a model that classifies multivariate ITS by explicitly seeking highly-relevant portions of an input series' timeline. CAT achieves this by integrating three components: (1) A Moment Network learns to seek relevant moments in an ITS's continuous timeline using reinforcement learning. (2) A Receptor Network models the temporal dynamics of both observations and their timing localized around predicted moments. (3) A recurrent Transition Model models the sequence of transitions between these moments, cultivating a representation with which the series is classified. Using synthetic and real data, we find that CAT outperforms ten state-of-the-art methods by finding short signals in long irregular time series.

==> figures/family_portrait.tex <==
\begin{figure}[tp]
    \centering
    
    \includegraphics[width=.45\textwidth]{figures/tall_novelty2.pdf}
    % \begin{subfigure}[t]{.57\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/fp_ram2.pdf}
    %     \caption{Attention-based classification \citep{mnih2014recurrent}}\label{fig:fp_ram}
    % \end{subfigure}
    % \begin{subfigure}[t]{.4\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/fp_ists2.pdf}
    %     \caption{ISTS classification \citep{shukla2019interpolation}}\label{fig:fp_ists}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.95\linewidth}
    %     \centering
    %     \vspace{3mm}
    %     \includegraphics[width=\textwidth]{figures/fp_cat2.pdf}
    %     \caption{Attention-based ISTS Classification (this paper)}\label{fig:fp_cat}
    % \end{subfigure}
    % % \caption{Comparing three classification problems. Traditional glimpse-based processing in (a) takes several glimpses of the input before classification. On the other hand, irregularly-sampled time series classification in (b) takes in the entire input time series and uses it for classification. The problem we study in (c) uses attention to process few, but relevant, moments in the time series for classification.}
    \caption{
    %Attention-based ISTS classification compared to ISTS classification and attention-based classification.
    Comparison of different classification problems. (a) Classification of Regular Time Series \cite{fawaz2019deep}; (b) Classification of Irregularly-Sampled Time Series \cite{shukla2019interpolation}; (c) Attention-based Classification of Image Data \cite{mnih2014recurrent}; (d) Attention-based Classification of Irregularly-Sampled Time Series (ours).
    }
    \label{fig:family_portrait}
    \vspace{-5mm}
\end{figure}

==> tables/accuracy_results.tex <==
% \begin{table*}[t]
% \centering
% \caption{Comparing the average Accuracy of all alternative algorithms. Parentheses indicate standard deviation.} \label{tab:accuracy}
% \vspace{-10pt}
% \begin{tabular}{lccccccccc}
% \toprule

% \multirow{2.25}{*}{\textbf{Datasets}} & \multicolumn{9}{c}{\textbf{Methods}}\\
% \cmidrule{2-10}
%                                 & RNN-interp
%                                 & RNN-mean
%                                 & RNN-$\Delta$t \cite{lipton2016directly}
%                                 & RNN-S \cite{lipton2016modeling}
%                                 & RNN-Decay \cite{mozer2017discrete}
%                                 & GRU-D \cite{che2018recurrent}
%                                 & IPN \cite{shukla2019interpolation}
%                                 & CAT-random
%                                 & CAT (ours)\\
% \midrule
% \textsc{UWave} & 0.75 (0.03) & 0.77 (0.01) & 0.76 (0.05) & 0.78 (0.01) & 0.75 (0.01) & -- & 0.73 (0.00) & 0.68 (0.00) & \textbf{0.92 (0.01)}\\
% \midrule
% \textsc{Walking} & 0.62 (0.04) & 0.59 (0.02) & 0.56 (0.02) & 0.61 (0.04) & 0.59 (0.02) & 0.63 (0.02) & 0.62 (0.01) & 0.61 (0.01) & \textbf{0.77 (0.03)}\\
% % \textsc{Sitting} & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \textsc{Running} & 0.52 (0.05) & 0.51 (0.09) & 0.48 (0.02) & 0.51 (0.07) & 0.51 (0.05) & 0.45 (0.01) & 0.46 (0.01) & 0.51 (0.01) & \textbf{0.53 (0.01)} \\
% % \textsc{ES-Bike} & -- & -- & -- & -- & -- & -- & -- & -- & --\\
% % \textsc{Sleeping} & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \textsc{LayingDown} & 0.78 (0.07) & 0.8 (0.04) & 0.83 (0.04) & \textbf{0.89 (0.02)} & 0.88 (0.05) & 0.82 (0.03) & 0.85 (0.05) & -- & \textbf{0.89 (0.03)}\\
% \bottomrule
% \end{tabular}\label{tab:extrasensory}
% \end{table*}

\begin{table*}[t]
\centering
\caption{Testing accuracy of all alternative algorithms. Parentheses denote standard deviation over all replications. Low Resolution denotes the use of 200 reference timesteps for all methods. High Resolution denotes the use of 500 reference timesteps.} \label{tab:accuracy}
\vspace{-10pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{clccccccccc}
\toprule

\multicolumn{2}{c}{\multirow{2.25}{*}{\textbf{Datasets}}} &  \multicolumn{9}{c}{\textbf{Methods}}\\
\cmidrule{3-11}
                                &
                                & RNN-interp
                                & RNN-mean
                                & RNN-$\Delta$t \cite{lipton2016directly}
                                & RNN-S \cite{lipton2016modeling}
                                & RNN-Decay \cite{mozer2017discrete}
                                & GRU-D \cite{che2018recurrent}
                                & IPN \cite{shukla2019interpolation}
                                & CAT-random
                                & CAT (ours)\\
\midrule
& \textsc{UWave} & 0.75 (0.03) & 0.77 (0.01) & 0.76 (0.05) & 0.78 (0.01) & 0.75 (0.01) & 0.81 (0.01) & 0.73 (0.00) & 0.68 (0.00) & \textbf{0.92 (0.01)}\\
\midrule
% \multirow{4}{*}{\rotatebox[origin=c]{90}{$\delta$=.001}}

% AKA 0.001 results
\multirow{4}{*}{\rotatebox[origin=c]{90}{\shortstack[c]{{Low}\\{Resolution}}}}
& \textsc{Walking} & 0.65 (0.02) & 0.64 (0.02) & 0.64 (0.01) & 0.64 (0.01) & 0.64 (0.02) & 
0.65 (0.01) & 0.65 (0.01) & 0.60 (0.02) & \textbf{0.74 (0.03)}  \\
% \textsc{Sitting} & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& \textsc{Running} & 0.52 (0.04) & 0.52 (0.09) & 0.52 (0.07) & 0.46 (0.03) & 0.44 (0.03) &
0.43 (0.01) & 0.46 (0.03) & 0.47 (0.01) & \textbf{0.54 (0.01)} \\
% \textsc{ES-Bike} & -- & -- & -- & -- & -- & -- & -- & -- & --\\
% \textsc{Sleeping} & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& \textsc{LyingDown} & 0.83 (0.05) & 0.78 (0.04) & 0.83 (0.04) & 0.82 (0.08) & 0.77 (0.04) & 0.78 (0.03) & 0.85 (0.04) & 0.76 (0.01) & \textbf{0.87 (0.04)}  \\
& \textsc{Sleeping} & 0.77 (0.07) & 0.85 (0.06) & 0.89 (0.05) & 0.90 (0.05) & 0.86 (0.02) & \textbf{0.92 (0.02)} & 0.85 (0.04) & 0.88 (0.01) & \textbf{0.91 (0.01)} \\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\shortstack[c]{{High}\\{Resolution}}}}
& \textsc{Walking} & 0.62 (0.04) & 0.59 (0.02) & 0.56 (0.02) & 0.61 (0.04) & 0.59 (0.02) & 0.63 (0.02) & 0.62 (0.01) & 0.61 (0.01) & \textbf{0.77 (0.03)}\\
% \textsc{Sitting} & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& \textsc{Running} & 0.52 (0.05) & 0.51 (0.09) & 0.48 (0.02) & 0.51 (0.07) & 0.51 (0.05) & 0.45 (0.01) & 0.46 (0.01) & 0.47 (0.00) & \textbf{0.54 (0.01)} \\
% \textsc{ES-Bike} & -- & -- & -- & -- & -- & -- & -- & -- & --\\
& \textsc{LyingDown} & 0.78 (0.07) & 0.8 (0.04) & 0.83 (0.04) & \textbf{0.89 (0.02)} & 0.88 (0.05) & 0.82 (0.03) & 0.85 (0.05) & 0.77 (0.00) & \textbf{0.89 (0.03)} \\
& \textsc{Sleeping} & 0.87 (0.06) & 0.89 (0.02) & 0.9 (0.03) & 0.9 (0.01) & 0.83 (0.06) & \textbf{0.91 (0.02)} & 0.86 (0.04) & 0.87 (0.01) & 0.9 (0.02) \\

% 0.002 results
% \midrule
% \multirow{4}{*}{\rotatebox[origin=c]{90}{$\delta$=.002}}
% & \textsc{Walking} & 0.72 (0.05) & 0.62 (0.01) & 0.64 (0.03) & 0.67 (0.01) & 0.65 (0.01) & 0.66 (0.02) & 0.67 (0.01) & -- & \textbf{0.73 (0.04)} \\
% % \textsc{Sitting} & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & \textsc{Running} & 0.49 (0.06) & 0.42 (0.03) & 0.42 (0.01) & 0.42 (0.00) & 0.42 (0.00) & 0.42 (0.01) & 0.45 (0.04) & -- & \textbf{0.49 (0.03)}\\
% % \textsc{ES-Bike} & -- & -- & -- & -- & -- & -- & -- & -- & --\\
% % \textsc{Sleeping} & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & \textsc{LyingDown} & 0.83 (0.03) & 0.83 (0.03) & 0.80 (0.05) & \textbf{0.89 (0.06)} & 0.76 (0.06) & 0.79 (0.04) & 0.84 (0.06) & -- & 0.83 (0.03) \\
% & \textsc{Sleeping} & 0.87 (0.04) & 0.86 (0.05) & 0.882 (0.05) & 0.91 (0.04) & 0.87 (0.05) & 0.90 (0.03) & 0.87 (0.04) & -- & \textbf{0.94 (0.01)} \\


% \midrule


\bottomrule
\end{tabular}\label{tab:main_results}
}
\end{table*}

% \begin{table*}[t]
% \centering
% \caption{Comparing the average Accuracy of all alternative algorithms. Parentheses indicate standard deviation.} \label{tab:accuracy}
% \vspace{-10pt}
% \begin{tabular}{clccccccc}
% \toprule

% \multirow{2.25}{*}{\textbf{Datasets}} & \multicolumn{9}{c}{\textbf{Methods}}\\
% \cmidrule{2-10}
%                                 & RNN-interp
%                                 & RNN-mean
%                                 & RNN-$\Delta$t \cite{lipton2016directly}
%                                 & RNN-S \cite{lipton2016modeling}
%                                 & RNN-Decay \cite{mozer2017discrete}
%                                 & GRU-D \cite{che2018recurrent}
%                                 & IPN \cite{shukla2019interpolation}
%                                 & CAT-random
%                                 & CAT (ours)\\
% \midrule
% & \textsc{UWave} & 0.75 (0.03) & 0.77 (0.01) & 0.76 (0.05) & 0.78 (0.01) & 0.75 (0.01) & -- & 0.73 (0.00) & 0.68 (0.00) & \textbf{0.92 (0.01)}\\
% \midrule
% \multirow{3}{*}{\rotatebox[origin=c]{90}{$\delta$=.001}}
% & \textsc{Walking} & 0.62 (0.04) & 0.59 (0.02) & 0.56 (0.02) & 0.61 (0.04) & 0.59 (0.02) & 0.63 (0.02) & 0.62 (0.01) & 0.61 (0.01) & \textbf{0.77 (0.03)}\\
% % \textsc{Sitting} & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & \textsc{Running} & 0.52 (0.05) & 0.51 (0.09) & 0.48 (0.02) & 0.51 (0.07) & 0.51 (0.05) & 0.45 (0.01) & 0.46 (0.01) & 0.51 (0.01) & \textbf{0.53 (0.01)} \\
% % \textsc{ES-Bike} & -- & -- & -- & -- & -- & -- & -- & -- & --\\
% % \textsc{Sleeping} & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & \textsc{LayingDown} & 0.78 (0.07) & 0.8 (0.04) & 0.83 (0.04) & \textbf{0.89 (0.02)} & 0.88 (0.05) & 0.82 (0.03) & 0.85 (0.05) & -- & \textbf{0.89 (0.03)}\\
% \midrule
% \multirow{3}{*}{\rotatebox[origin=c]{90}{$\delta$=.002}}
% & \textsc{Walking} & 0.62 (0.04) & 0.59 (0.02) & 0.56 (0.02) & 0.61 (0.04) & 0.59 (0.02) & 0.63 (0.02) & 0.62 (0.01) & 0.61 (0.01) & \textbf{0.77 (0.03)}\\
% % \textsc{Sitting} & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & \textsc{Running} & 0.52 (0.05) & 0.51 (0.09) & 0.48 (0.02) & 0.51 (0.07) & 0.51 (0.05) & 0.45 (0.01) & 0.46 (0.01) & 0.51 (0.01) & \textbf{0.53 (0.01)} \\
% % \textsc{ES-Bike} & -- & -- & -- & -- & -- & -- & -- & -- & --\\
% % \textsc{Sleeping} & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% & \textsc{LayingDown} & 0.78 (0.07) & 0.8 (0.04) & 0.83 (0.04) & \textbf{0.89 (0.02)} & 0.88 (0.05) & 0.82 (0.03) & 0.85 (0.05) & -- & \textbf{0.89 (0.03)}\\

% \bottomrule
% \end{tabular}\label{tab:extrasensory}
% \end{table*}

==> tables/high_res.tex <==
\begin{table*}[t]
\centering
% \vspace{-10pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2.25}{*}{\textbf{Data}} &  \multicolumn{12}{c}{\textbf{Method}}\\
\cmidrule{2-13}

\midrule
GRU-interp & 0.62 (0.04) 	 & 0.52 (0.05) 	 & 0.78 (0.07) 	 & 0.76 (0.05) \\
GRU-mean & 0.59 (0.02) 	 & 0.51 (0.09) 	 & 0.8 (0.04) 	 & 0.79 (0.02) \\
GRU-$\Delta$t \cite{lipton2016directly} & 0.56 (0.02) 	 & 0.48 (0.02) 	 & 0.83 (0.04) 	 & 0.80 (0.03) \\
GRU-S \cite{lipton2016modeling} & 0.61 (0.04) 	 & 0.51 (0.07) 	 & \textbf{0.89 (0.02)} 	 & 0.80 (0.02) \\
GRU-Decay \cite{mozer2017discrete} & 0.59 (0.02) 	 & 0.51 (0.05) 	 & 0.88 (0.05) 	 & 0.77 (0.02) \\
GRU-D \cite{che2018recurrent} & 0.63 (0.02) 	 & 0.45 (0.01) 	 & 0.82 (0.03) 	 & 0.73 (0.01) \\
IPN \cite{shukla2019interpolation} & 0.62 (0.01) 	 & 0.46 (0.01) 	 & 0.85 (0.05) 	 & 0.78 (0.04) \\
TF \cite{vaswani2017attention} & 0.69	& 0.61	& 0.72	0.62\\
mTAN \cite{shukla2021multi} & 0.64 (0.01) 	 & \textbf{0.55 (0.01)} 	 & 0.74 (0.02) 	 & 0.76 (0.02)\\ 
NCDE \cite{kidger2020neural} & 0.66	& 0.53	& 0.75	& 0.71\\
CAT-random & 0.61 (0.01) 	 & 0.47 (0.00) 	 & 0.77 (0.00) 	 & 0.74 (0.01) \\
CAT (ours)\\ & \textbf{0.83 (0.03)}	 & \textbf{0.54 (0.01)} 	 & \textbf{0.89 (0.03)} & \textbf{0.90 (0.01)}\\
 
% \textsc{Sleeping} & 0.87 (0.06) & 0.89 (0.02) & 0.9 (0.03) & 0.9 (0.01) & 0.83 (0.06) & \textbf{0.91 (0.02)} & 0.86 (0.04) & 0.87 (0.01) & 0.9 (0.02) \\
\bottomrule
\end{tabular}
}
% \vspace{-9pt}
\caption{Testing accuracy of all methods with \textit{frequently}-imputed values for the Human Activity Recognition Datasets.}\label{tab:high_res}
\end{table*}

==> tables/low_res.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2.25}{*}{\textbf{Data}} &  \multicolumn{12}{c}{\textbf{Methods}}\\
\cmidrule{2-13}
                                & GRU-interp
                                & GRU-mean
                                & GRU-$\Delta$t \cite{lipton2016directly}
                                & GRU-S \cite{lipton2016modeling}
                                & GRU-Decay \cite{mozer2017discrete}
                                & GRU-D \cite{che2018recurrent}
                                & IPN \cite{shukla2019interpolation}
                                & TF \cite{vaswani2017attention}
                                & mTAN \cite{shukla2021multi}
                                & NCDE \cite{kidger2020neural}
                                & CAT-random
                                & CAT (ours)\\
\midrule
\textsc{Walking} & 0.65 (0.02) & 0.64 (0.02) & 0.64 (0.01) & 0.64 (0.01) & 0.64 (0.02) & 0.65 (0.01) & 0.65 (0.01) & 0.78 & 0.68 (0.02) & 0.66 & 0.60 (0.02) & \textbf{0.81 (0.03)}  \\
\textsc{Running} & 0.52 (0.04) & 0.52 (0.09) & 0.52 (0.07) & 0.46 (0.03) & 0.44 (0.03) & 0.43 (0.01) & 0.46 (0.03) & 0.48 & 0.56 (0.01) & 0.53 & 0.47 (0.01) & \textbf{0.62 (0.01)} \\
\textsc{Lying} & 0.83 (0.05) & 0.78 (0.04) & 0.83 (0.04) & 0.82 (0.08) & 0.77 (0.04) & 0.78 (0.03) & 0.85 (0.04) & 0.76 & 0.73 (0.00) & 0.75 & 0.76 (0.01) & \textbf{0.87 (0.04)}  \\
\textsc{Sleeping} & 0.76 (0.05) & 0.79 (0.01) & 0.79 (0.03) & 0.76 (0.03) & 0.78 (0.03) & 0.76 (0.03) & 0.77 (0.03) & 0.8 & 0.76 (0.02) & 0.71 & 0.73 (0.01) & \textbf{0.91 (0.02)}  \\
% \textsc{Sleeping} & 0.77 (0.07) & 0.85 (0.06) & 0.89 (0.05) & 0.90 (0.05) & 0.86 (0.02) & \textbf{0.92 (0.02)} & 0.85 (0.04) & 0.88 (0.01) & \textbf{0.91 (0.01)} \\
\bottomrule
\end{tabular}
}
% \vspace{-9pt}
\caption{Testing accuracy of all methods with \textit{infrequently}-imputed values for the Human Activity Recognition Datasets.}\label{tab:low_res}
\end{table*}


==> tex/commands.tex <==
% COMMANDS:
% - bigmid: Dynamically sized mid bar.
% - spacerule: add a centered dashed line with space above and below
% - \dbox{#1}: Adds a nicely formatted slightly grey box around #1
% - \begin{dproof} ... \end{dproof}: A nicely formatted proof. Use \qedhere to place qed
% - \ddef{#1}{#2}: Makes a definition (and counts defs). #1 goes inside parens at beginning, #2 is actual def.
% - \begin{dtable}{#1} ... \end{dtable}: Makes a minimalist table. #1 is the alignment, for example: {clrr} would be a 4 column, center left right right table.

\newcommand{\peq}{\mathrel{{+}{=}}}

% Dynamically sized mid bar.
\newcommand{\bigmid}{\mathrel{\Big|}}

% ---- Nice Color Palette and Notes ----
%\definecolor{tblue}{RGB}{94, 129, 172}
\definecolor{tblue}{RGB}{93, 142, 150}
\definecolor{tred}{RGB}{191, 97, 106}
%\definecolor{tblue}{RGB}{98, 140, 190}
\definecolor{dlblue}{RGB}{216, 235, 255}
\definecolor{dgreen}{RGB}{124, 155, 127}
\definecolor{dpink}{RGB}{207, 166, 208}
\definecolor{dyellow}{RGB}{255, 248, 199}
\definecolor{dgray}{RGB}{46, 49, 49}

% TODO
\newcommand{\todo}[1]{\textcolor{tred}{TODO: #1}}
\newcommand{\tnote}[1]{\textcolor{tblue}{#1 -tom}}
\definecolor{cred}{RGB}{191, 97, 106}
\newcommand{\cnote}[1]{\textcolor{cred}{#1 -cansu}}

% URL
\newcommand{\durl}[1]{\textcolor{tblue}{\underline{\url{#1}}}}

% Circled Numbers
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=0.7pt] (char) {\footnotesize{#1}};}}
% From: http://tex.stackexchange.com/questions/7032/good-way-to-make-textcircled-numbers

% Under set numbered subset of equation
\newcommand{\numeq}[3]{\underset{\textcolor{#2}{\circled{#1}}}{\textcolor{#2}{#3}}}

% ---- Abbreviations -----
\newcommand{\tc}[2]{\textcolor{#1}{#2}}
\newcommand{\ubr}[1]{\underbrace{#1}}
\newcommand{\uset}[2]{\underset{#1}{#2}}
\newcommand{\eps}{\varepsilon}

% Typical limit:
\newcommand{\nlim}{\underset{n \rightarrow \infty}{\lim}}
\newcommand{\nsum}{\sum_{i = 1}^n}
\newcommand{\nprod}{\prod_{i = 1}^n}

% Add an hrule with some space
\newcommand{\spacerule}{\begin{center}\hdashrule{2cm}{1pt}{1pt}\end{center}}

% Mathcal and Mathbb
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\indic}{\mathbbm{1}}
\newcommand{\bE}{\mathbb{E}}

\newcommand{\ra}{\rightarrow}
\newcommand{\la}{\leftarrow}

% ---- Figures, Boxes, Theorems, Etc. ----

% Basic Image
\newcommand{\img}[2]{
\begin{center}
\includegraphics[scale=#2]{#1}
\end{center}}

% Put a fancy box around things.
\newcommand{\dbox}[1]{
\begin{mdframed}[roundcorner=4pt, backgroundcolor=gray!5]
\vspace{1mm}
{#1}
\end{mdframed}
}

%  --- PROOFS ---

% Inner environment for Proofs
\newmdenv[
  topline=false,
  bottomline=false,
  rightline = false,
  leftmargin=10pt,
  rightmargin=0pt,
  innertopmargin=0pt,
  innerbottommargin=0pt
]{innerproof}

% Proof Command
\newenvironment{dproof}[1][Proof]{\begin{proof}[#1] \text{\vspace{2mm}} \begin{innerproof}}{\end{innerproof}\end{proof}\vspace{4mm}}

% Quick Definition
\newcounter{DaveDefCounter}
\setcounter{DaveDefCounter}{1}

\newcommand{\ddef}[2]
{
\begin{mdframed}[roundcorner=1pt, backgroundcolor=white]
\vspace{1mm}
{\bf Definition \theDaveDefCounter} (#1): {\it #2}
\stepcounter{DaveDefCounter}
\end{mdframed}
}

% Block Quote
\newenvironment{dblockquote}[2]{
\begin{blockquote}
#2
\vspace{-2mm}\hspace{10mm}{#1} \\
\end{blockquote}}

% Algorithm
\newenvironment{dalg}[1]
{\begin{algorithm}\caption{#1}\begin{algorithmic}}
{\end{algorithmic}\end{algorithm}}


% Quick Table
\newenvironment{dtable}[1]
{\begin{figure}[h]
\centering
\begin{tabular}{#1}\toprule}
{\bottomrule
\end{tabular}
\end{figure}}

% For numbering the last of an align*
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}


==> tex/full_bib.tex <==
% --- Datasets ---

@inproceedings{hartvigsen2018early,
  title={Early Prediction of MRSA Infections using Electronic Health Records},
  author={Hartvigsen, Thomas and Sen, Cansu and Brownell, Sarah and Teeple, Erin and Kong, Xiangnan and Rundensteiner, Elke A},
  booktitle={HEALTHINF},
  pages={156--167},
  year={2018}
}

@article{gupta2020early,
  title={An Early Classification Approach for Multivariate Time Series of On-Vehicle Sensors in Transportation},
  author={Gupta, Ashish and Gupta, Hari Prabhat and Biswas, Bhaskar and Dutta, Tanima},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  year={2020},
  publisher={IEEE}
}

@inproceedings{brunskill2013sample,
  title={Sample complexity of multi-task reinforcement learning},
  author={Brunskill, Emma and Li, Lihong},
  booktitle={UAI},
  pages={122--131},
  year={2013}
}

@article{silver2016mastering,
  title={Mastering the game of Go with deep neural networks and tree search},
  author={Silver, David and Huang, Aja and Maddison, Chris J and Guez, Arthur and Sifre, Laurent and Van Den Driessche, George and Schrittwieser, Julian and Antonoglou, Ioannis and Panneershelvam, Veda and Lanctot, Marc and others},
  journal={nature},
  volume={529},
  number={7587},
  pages={484},
  year={2016},
  publisher={Nature Publishing Group}
}

@article{mnih2013playing,
  title={Playing atari with deep reinforcement learning},
  author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Graves, Alex and Antonoglou, Ioannis and Wierstra, Daan and Riedmiller, Martin},
  journal={arXiv preprint arXiv:1312.5602},
  year={2013}
}

@article{vaizman2017recognizing,
  title={Recognizing detailed human context in the wild from smartphones and smartwatches},
  author={Vaizman, Yonatan and Ellis, Katherine and Lanckriet, Gert},
  journal={IEEE Pervasive Computing},
  volume={16},
  number={4},
  pages={62--74},
  year={2017},
  publisher={IEEE}
}

@inproceedings{anguita2013public,
  title={A public domain dataset for human activity recognition using smartphones.},
  author={Anguita, Davide and Ghio, Alessandro and Oneto, Luca and Parra, Xavier and Reyes-Ortiz, Jorge Luis},
  booktitle={ESANN},
  year={2013}
}

@article{briggs2012acoustic,
  title={Acoustic classification of multiple simultaneous bird species: A multi-instance multi-label approach},
  author={Briggs, Forrest and Lakshminarayanan, Balaji and Neal, Lawrence and Fern, Xiaoli Z and Raich, Raviv and Hadley, Sarah JK and Hadley, Adam S and Betts, Matthew G},
  journal={The Journal of the Acoustical Society of America},
  volume={131},
  number={6},
  pages={4640--4650},
  year={2012},
  publisher={Acoustical Society of America}
}


% --- Multi-label Learning ---
@inproceedings{nam2019learning,
  title={Learning Context-dependent Label Permutations for Multi-label Classification},
  author={Nam, Jinseok and Kim, Young-Bum and Mencia, Eneldo Loza and Park, Sunghyun and Sarikaya, Ruhi and F{\"u}rnkranz, Johannes},
  booktitle={ICML},
  pages={4733--4742},
  year={2019}
}

@inproceedings{fujita2019end,
  title={End-to-End Neural Speaker Diarization with Permutation-Free Objectives},
  author={Fujita, Yusuke and Kanda, Naoyuki and Horiguchi, Shota and Nagamatsu, Kenji and Watanabe, Shinji},
  booktitle={Interspeech},
  year={2019}
}

@inproceedings{yang2018sgm,
  title={SGM: Sequence Generation Model for Multi-label Classification},
  author={Yang, Pengcheng and Sun, Xu and Li, Wei and Ma, Shuming and Wu, Wei and Wang, Houfeng},
  booktitle={COLING},
  pages={3915--3926},
  year={2018}
}

@inproceedings{vinyals2015order,
  title={Order matters: Sequence to sequence for sets},
  author={Vinyals, Oriol and Bengio, Samy and Kudlur, Manjunath},
  booktitle={ICLR},
  year={2017}
}

@inproceedings{nam2017maximizing,
  title={Maximizing subset accuracy with recurrent neural networks in multi-label classification},
  author={Nam, Jinseok and Menc{\'\i}a, Eneldo Loza and Kim, Hyunwoo J and F{\"u}rnkranz, Johannes},
  booktitle={NeurIPS},
  pages={5413--5423},
  year={2017}
}

@inproceedings{chen2018order,
  title={Order-free RNN with visual attention for multi-label classification},
  author={Chen, Shang-Fu and Chen, Yi-Chen and Yeh, Chih-Kuan and Wang, Yu-Chiang Frank},
  booktitle={AAAI},
  year={2018}
}

@inproceedings{wang2016cnn,
  title={Cnn-rnn: A unified framework for multi-label image classification},
  author={Wang, Jiang and Yang, Yi and Mao, Junhua and Huang, Zhiheng and Huang, Chang and Xu, Wei},
  booktitle={CVPR},
  pages={2285--2294},
  year={2016}
}

@article{yao2017learning,
  title={Learning to diagnose from scratch by exploiting dependencies among labels},
  author={Yao, Li and Poblenz, Eric and Dagunts, Dmitry and Covington, Ben and Bernard, Devon and Lyman, Kevin},
  journal={arXiv preprint arXiv:1710.10501},
  year={2017}
}

@inproceedings{tsai2020order,
  title={Order-free Learning Alleviating Exposure Bias in Multi-label Classification},
  author={Tsai, Che-Ping and Lee, Hung-Yi},
  booktitle={AAAI},
  year={2020}
}


% --- Early Classification ---
@inproceedings{dennis2018multiple,
  title={Multiple instance learning for efficient sequential data classification on resource-constrained devices},
  author={Dennis, Don and Pabbaraju, Chirag and Simhadri, Harsha Vardhan and Jain, Prateek},
  booktitle={NeurIPS},
  pages={10953--10964},
  year={2018}
}

@article{martinez2019adaptive,
  title={Adaptive early classification of temporal sequences using deep reinforcement learning},
  author={Martinez, Coralie and Ramasso, Emmanuel and Perrin, Guillaume and Rombaut, Mich{\`e}le},
  journal={Knowledge-Based Systems},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{wiens2012patient,
  title={Patient risk stratification for hospital-associated c. diff as a time-series classification task},
  author={Wiens, Jenna and Horvitz, Eric and Guttag, John V},
  booktitle={NeurIPS},
  pages={467--475},
  year={2012}
}

@incollection{sutton2000policy,
  title={Policy gradient methods for reinforcement learning with function approximation},
  author={Sutton, Richard S and McAllester, David A and Singh, Satinder P and Mansour, Yishay},
  booktitle={NeurIPS},
  pages={1057--1063},
  year={2000}
}

@incollection{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  booktitle={ICLR},
  year={2014}
}


@incollection{schulman2015gradient,
  title={Gradient estimation using stochastic computation graphs},
  author={Schulman, John and Heess, Nicolas and Weber, Theophane and Abbeel, Pieter},
  booktitle={NeurIPS},
  pages={3528--3536},
  year={2015}
}

@inproceedings{xu2015show,
  title={Show, attend and tell: Neural image caption generation with visual attention},
  author={Xu, Kelvin and Ba, Jimmy and Kiros, Ryan and Cho, Kyunghyun and Courville, Aaron and Salakhudinov, Ruslan and Zemel, Rich and Bengio, Yoshua},
  booktitle={ICML},
  pages={2048--2057},
  year={2015}
}

@misc{graves2013generating,
  title={Generating sequences with recurrent neural networks},
  author={Graves, Alex},
  journal={arXiv preprint arXiv:1308.0850},
  year={arXiv, 2013}
}

@inproceedings{mikolov2010recurrent,
  title={Recurrent neural network based language model},
  author={Mikolov, Tom{\'a}{\v{s}} and Karafi{\'a}t, Martin and Burget, Luk{\'a}{\v{s}} and {\v{C}}ernock{\`y}, Jan and Khudanpur, Sanjeev},
  booktitle={ISCA},
  year={2010}
}

@inproceedings{graves2013speech,
  title={Speech recognition with deep recurrent neural networks},
  author={Graves, Alex and Mohamed, Abdel-rahman and Hinton, Geoffrey},
  booktitle={IEEE ICASSP},
  pages={6645--6649},
  year={2013}
}

@misc{cirecsan2012multi,
  title={Multi-column deep neural networks for image classification},
  author={Cire{\c{s}}an, Dan and Meier, Ueli and Schmidhuber, J{\"u}rgen},
  journal={arXiv preprint arXiv:1202.2745},
  year={arXiv, 2012}
}

@article{elman1990finding,
  title={Finding structure in time},
  author={Elman, Jeffrey L},
  journal={Cognitive science},
  volume={14},
  number={2},
  pages={179--211},
  year={1990},
  publisher={Wiley Online Library}
}

@article{bengio1994learning,
  title={Learning long-term dependencies with gradient descent is difficult},
  author={Bengio, Yoshua and Simard, Patrice and Frasconi, Paolo},
  journal={IEEE Transactions on Neural Networks},
  volume={5},
  number={2},
  pages={157--166},
  year={1994}
}

@inproceedings{ye2009time,
  title={Time series shapelets: a new primitive for data mining},
  author={Ye, Lexiang and Keogh, Eamonn},
  booktitle={ACM SIGKDD},
  pages={947--956},
  year={2009}
}

@inproceedings{mnih2014recurrent,
  title={Recurrent models of visual attention},
  author={Mnih, Volodymyr and Heess, Nicolas and Graves, Alex and Kavukcuoglu, Koray},
  booktitle={NeurIPS},
  pages={2204--2212},
  year={2014}
}

@article{parrish2013classifying,
  title={Classifying with confidence from incomplete information},
  author={Parrish, Nathan and Anderson, Hyrum S and Gupta, Maya R and Hsiao, Dun Yu},
  journal={Journal of Machine Learning Research},
  volume={14},
  number={1},
  pages={3561--3589},
  year={2013}
}

@inproceedings{lin2015reliable,
  title={Reliable early classification on multivariate time series with numerical and categorical attributes},
  author={Lin, Yu-Feng and Chen, Hsuan-Hsu and Tseng, Vincent S and Pei, Jian},
  booktitle={PAKDD},
  pages={199--211},
  year={2015}
}

@misc{srivastava2015highway,
  title={Highway networks},
  author={Srivastava, Rupesh Kumar and Greff, Klaus and Schmidhuber, J{\"u}rgen},
  journal={arXiv preprint arXiv:1505.00387},
  year={arXiv, 2015}
}

@article{bengio2015conditional,
  title={Conditional computation in neural networks for faster models},
  author={Bengio, Emmanuel and Bacon, Pierre-Luc and Pineau, Joelle and Precup, Doina},
  journal={arXiv preprint arXiv:1511.06297},
  year={arXiv, 2015}
}


@inproceedings{huang2017length,
  title={Length Adaptive Recurrent Model for Text Classification},
  author={Huang, Zhengjie and Ye, Zi and Li, Shuangyin and Pan, Rong},
  booktitle={CIKM},
  pages={1019--1027},
  year={2017}
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural Computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997}
}

@article{he2015early,
  title={Early classification on multivariate time series},
  author={He, Guoliang and Duan, Yong and Peng, Rong and Jing, Xiaoyuan and Qian, Tieyun and Wang, Lingling},
  journal={Neurocomputing},
  volume={149},
  pages={777--787},
  year={2015}
}

@inproceedings{xing2011extracting,
  title={Extracting interpretable features for early classification on time series},
  author={Xing, Zhengzheng and Pei, Jian and Yu, Philip S and Wang, Ke},
  booktitle={SDM},
  pages={247--258},
  year={2011}
}

@article{xing2012early,
  title={Early classification on time series},
  author={Xing, Zhengzheng and Pei, Jian and Yu, Philip S},
  journal={Knowledge and Information Systems},
  volume={31},
  number={1},
  pages={105--127},
  year={2012}
}

@inproceedings{xing2009early,
  title={Early Prediction on Time Series: A Nearest Neighbor Approach},
  author={Xing, Zhengzheng and Pei, Jian and Yu, Phillip},
  booktitle={IJCAI},
  pages={1297--1302},
  year={2009}
}


@article{johnson2016mimic,
  title={MIMIC-III, a freely accessible critical care database},
  author={Johnson, Alistair EW and Pollard, Tom J and Shen, Lu and Lehman, Li-wei H and Feng, Mengling and Ghassemi, Mohammad and Moody, Benjamin and Szolovits, Peter and Celi, Leo Anthony and Mark, Roger G},
  journal={Scientific Data},
  volume={3},
  year={2016}
}

@article{shortreed2011informing,
  title={Informing sequential clinical decision-making through reinforcement learning: an empirical study},
  author={Shortreed, Susan M and Laber, Eric and Lizotte, Daniel J and Stroup, T Scott and Pineau, Joelle and Murphy, Susan A},
  journal={Machine Learning},
  volume={84},
  number={1-2},
  pages={109--136},
  year={2011}
}

@article{williams1992simple,
  title={Simple statistical gradient-following algorithms for connectionist reinforcement learning},
  author={Williams, Ronald J},
  journal={Machine Learning},
  volume={8},
  number={3-4},
  pages={229--256},
  year={1992}
}

@inproceedings{karlsson2016early,
  title={Early Random Shapelet Forest},
  author={Karlsson, Isak and Papapetrou, Panagiotis and Bostr{\"o}m, Henrik},
  booktitle={International Conference on Discovery Science},
  pages={261--276},
  year={2016}
}

@article{ghalwash2012early,
  title={Early classification of multivariate temporal observations by extraction of interpretable shapelets},
  author={Ghalwash, Mohamed F and Obradovic, Zoran},
  journal={BMC Bioinformatics},
  volume={13},
  number={1},
  pages={195},
  year={2012}
}

@inproceedings{guez2008adaptive,
  title={Adaptive Treatment of Epilepsy via Batch-mode Reinforcement Learning.},
  author={Guez, Arthur and Vincent, Robert D and Avoli, Massimo and Pineau, Joelle},
  booktitle={AAAI},
  pages={1671--1678},
  year={2008}
}

@inproceedings{lizotte2010efficient,
  title={Efficient reinforcement learning with multiple reward functions for randomized controlled trial analysis},
  author={Lizotte, Daniel J and Bowling, Michael H and Murphy, Susan A},
  booktitle={ICML},
  pages={695--702},
  year={2010}
}

@techreport{lizotte2009assessing,
  title={Assessing confidence in policies learned from sequential randomized trials},
  author={Lizotte, Daniel J and Laber, Eric and Murphy, Susan A},
  year={2009},
  institution={Technical Report, Department of Statistics, University of Michigan, Ann Arbor, Michigan}
}

@article{pineau2007constructing,
  title={Constructing evidence-based treatment strategies using methods from computer science},
  author={Pineau, Joelle and Bellemare, Marc G and Rush, A John and Ghizaru, Adrian and Murphy, Susan A},
  journal={Drug and Alcohol Dependence},
  volume={88},
  pages={S52--S60},
  year={2007},
  publisher={Elsevier}
}

@inproceedings{li2014early,
  title={Early classification of ongoing observation},
  author={Li, Kang and Li, Sheng and Fu, Yun},
  booktitle={ICDM},
  pages={310--319},
  year={2014}
}

@article{mori2017reliable,
  title={Reliable early classification of time series based on discriminating the classes over time},
  author={Mori, Usue and Mendiburu, Alexander and Keogh, Eamonn and Lozano, Jose A},
  journal={Data Mining and Knowledge Discovery},
  volume={31},
  number={1},
  pages={233--263},
  year={2017}
}

@article{sen2017crest,
title={CREST - Risk Prediction for Clostridium Difficile Infection Using Multimodal Data Mining},
author={Sen, Cansu and Hartvigsen, Thomas and Rundensteiner, Elke and Claypool, Kajal},
journal={Machine Learning and Knowledge Discovery in Databases},
pages = {49-60},
year={2017}}


@inproceedings{ma2016learning,
  title={Learning activity progression in lstms for activity detection and early detection},
  author={Ma, Shugao and Sigal, Leonid and Sclaroff, Stan},
  booktitle={CVPR},
  pages={1942--1950},
  year={2016}
}

@inproceedings{cho2014learning,
  title={Learning phrase representations using RNN encoder-decoder for statistical machine translation},
  author={Cho, Kyunghyun and Van Merri{\"e}nboer, Bart and Gulcehre, Caglar and Bahdanau, Dzmitry and Bougares, Fethi and Schwenk, Holger and Bengio, Yoshua},
  booktitle={EMNLP},
  pages={1724--1734},
  year={2014}
}

@inproceedings{weber2014lstm,
  title={Lstm-based early recognition of motion patterns},
  author={Weber, Markus and Liwicki, Marcus and Stricker, Didier and Scholzel, Christopher and Uchida, Seiichi},
  booktitle={ICPR},
  pages={3552--3557},
  year={2014},
  organization={IEEE}
}

@misc{graves2016adaptive,
  title={Adaptive computation time for recurrent neural networks},
  author={Graves, Alex},
  journal={arXiv preprint arXiv:1603.08983},
  year={arXiv, 2016},
}

@misc{bengio2013estimating,
  title={Estimating or propagating gradients through stochastic neurons for conditional computation},
  author={Bengio, Yoshua and L{\'e}onard, Nicholas and Courville, Aaron},
  journal={arXiv preprint arXiv:1308.3432},
  year={arXiv, 2013}
}

@misc{schmidhuber2012self,
  title={Self-delimiting neural networks},
  author={Schmidhuber, J{\"u}rgen},
  journal={arXiv preprint arXiv:1210.0118},
  year={arXiv, 2012}
}

@inproceedings{keogh2006intelligent,
  title={Intelligent icons: Integrating lite-weight data mining and visualization into GUI operating systems},
  author={Keogh, Eamonn and Wei, Li and Xi, Xiaopeng and Lonardi, Stefano and Shieh, Jin and Sirowy, Scott},
  booktitle={ICDM},
  pages={912--916},
  year={2006}
}

@inproceedings{bridle1990training,
  title={Training stochastic model recognition algorithms as networks can lead to maximum mutual information estimation of parameters},
  author={Bridle, John S},
  booktitle={NeurIPS},
  year={1990}
}

@inproceedings{ghalwash2013extraction,
  title={Extraction of interpretable multivariate patterns for early diagnostics},
  author={Ghalwash, Mohamed F and Radosavljevic, Vladan and Obradovic, Zoran},
  booktitle={ICDM},
  pages={201--210},
  year={2013}
}

@inproceedings{ghalwash2014utilizing,
  title={Utilizing temporal patterns for estimating uncertainty in interpretable early decision making},
  author={Ghalwash, Mohamed F and Radosavljevic, Vladan and Obradovic, Zoran},
  booktitle={SIGKDD},
  pages={402--411},
  year={2014},
}

@article{andrzejak2001indications,
  title={Indications of nonlinear deterministic and finite-dimensional structures in time series of brain electrical activity: Dependence on recording region and brain state},
  author={Andrzejak, Ralph G and Lehnertz, Klaus and Mormann, Florian and Rieke, Christoph and David, Peter and Elger, Christian E},
  journal={Physical Review E},
  volume={64},
  number={6},
  pages={061907},
  year={2001},
  publisher={APS}
}

@inproceedings{kawala2013predictions,
  title={Pr{\'e}dictions d'activit{\'e} dans les r{\'e}seaux sociaux en ligne},
  author={Kawala, Fran{\c{c}}ois and Douzal-Chouakria, Ahlame and Gaussier, Eric and Dimert, Eustache},
  booktitle={4i{\`e}me conf{\'e}rence sur les mod{\`e}les et l'analyse des r{\'e}seaux: Approches math{\'e}matiques et informatiques},
  pages={16},
  year={2013}
}

@article{mori2018early,
  title={Early classification of time series by simultaneously optimizing the accuracy and earliness},
  author={Mori, Usue and Mendiburu, Alexander and Dasgupta, Sanjoy and Lozano, Jose A},
  journal={IEEE transactions on neural networks and learning systems},
  volume={29},
  number={10},
  pages={4569 -- 4578},
  year={2018},
  publisher={IEEE}
}

@inproceedings{coralie2018deep,
  title={A deep reinforcement learning approach for early classification of time series},
  author={Coralie, Martinez and Perrin, Guillaume and Ramasso, E and Rombaut Mich{\`e}lle},
  booktitle={EUSIPCO},
  year={2018}
}

@inproceedings{hartvigsen2019adaptive,
  title={Adaptive-Halting Policy Network for Early Classification},
  author={Hartvigsen, Thomas and Sen, Cansu and Kong, Xiangnan and Rundensteiner, Elke},
  booktitle={SIGKDD},
  pages={101--110},
  year={2019}
}


@article{BLS04,
  title={Learning multi-label scene classification},
  author    = {Matthew R. Boutell and
               Jiebo Luo and
               Xipeng Shen and
               Christopher M. Brown},
  journal={Pattern Recognition},
  volume={37},
  number={9},
  pages={1757 -- 1771},
  year={2004}
}


@article{ZJL20,
  title={Multi-label Prediction in Time Series Data using Deep Neural Networks},
  author    = {Wenyu Zhang and
               Devesh K. Jha and
               Emil Laftchiev and
               Daniel Nikovski},
  title     = {Multi-label Prediction in Time Series Data using Deep Neural Networks},
  journal   = {arXiv preprint},
  volume    = {abs/2001.10098},
  year      = {2020}
}

==> tex/header.tex <==
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{wrapfig}
\usepackage{amsmath,amsfonts}
\usepackage{dsfont}
\usepackage{fancyvrb}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{subcaption}
\usepackage{setspace}
\usepackage{pifont}
\usepackage{enumitem}
\usepackage{xcolor}
\usepackage{graphics}
\usepackage{svg}
\usepackage{dblfloatfix}
\usepackage{float}
\usepackage{amsthm}
\usepackage{algorithmic}
\usepackage[ruled,vlined]{algorithm2e}
\SetKwComment{Comment}{\# }{}

\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]

\graphicspath{{images/}}

\newcommand{\ie}[0]{\textit{i.e.},\ }
\newcommand{\eg}[0]{\textit{e.g.},\ }
\newcommand{\etc}[0]{\textit{etc.}\ }

\pagestyle{plain} % display page numbers
% Sorry, I was experimenting with this -tom
